RECAST: Expanding the Boundaries of LLMs' Complex Instruction Following with Multi-Constraint Data

Large language models (LLMs) are increasingly expected to tackle complex tasks, driven by their expanding applications and users' growing proficiency in crafting sophisticated prompts. However, as the number of explicitly stated requirements increases (particularly more than 10 constraints), LLMs often struggle to accurately follow such complex instructions, which limits their applicability in complex real-world scenarios. To the best of our knowledge, existing datasets do not exceed 10 constraints per instance. To address this challenge, we propose RECAST, an efficient and scalable framework for synthesizing datasets where each example incorporates far more constraints than those in existing benchmarks, aiming to challenge and extend the boundaries of models' ability to follow complex instructions. These constraints are extracted from real-world prompt-response pairs to ensure practical relevance. Using this framework, we construct RECAST-30K, a large-scale, high-quality dataset comprising 30k instances spanning 19 constraint types. Experimental results demonstrate that models finetuned on RECAST-30K substantially improve in following complex instructions while maintaining their general capabilities without degradation. Moreover, RECAST enables automatic verification of constraint satisfaction via rule-based validators for quantitative constraints and LLM-based validators for qualitative ones; the verifiability provided by RECAST enables the design of reward functions for reinforcement learning, which further boosts model performance on complex and challenging tasks.

==> iclr2026/draft.tex <==
%nips版本的Introduction
\section{Introduction}

Large language models (LLMs) have demonstrated remarkable capabilities in solving various NLP tasks \cite{math_survey,creative_writing2,creative_writing1,reasoning_survey,code_survey,llmwriting,code_survey2} and are widely used in practical scenarios \cite{judge_survey,roleplay,legal_survey,medicine_survey}.
However, they still struggle with complex multi-constraint scenarios that are prevalent in real-world applications, 
such as constitutional AI systems requiring adherence to multiple principles simultaneously \cite{constitutional_ai,inverse_constitutional_ai,s_constitutional,c3ai}, and enterprise assistants managing detailed business rules \cite{de2025automated, grohs2023large, Giorgio_Conversation}.
Recently, LLM-based autonomous agents have attracted increasing attention from both academia and industry. Surveys such as \cite{wang2024survey} highlight their tremendous potential in social sciences, natural sciences, and engineering, which fundamentally relies on the ability of LLMs to follow complex instructions.
As shown in Figure \ref{fig:example}, when instruction complexity increases, with multiple explicit constraints in a single prompt, even advanced models like GPT-4o \cite{gpt4} show marked performance degradation, which has been emphasized in multiple benchmarks \cite{ferraz2024llm, jiang2023followbench, infobench, wen2024benchmarking}.
Therefore, advancing the complex instruction-following capabilities of LLMs is crucial for promoting their practical deployment.
Although prior studies have explored methods to evaluate and improve the instruction-following abilities of LLMs, existing research remains limited in scope. Works such as \cite{jiang2023followbench} and \cite{wen2024benchmarking} evaluated LLMs’ instruction-following performance and explored the use of LLMs themselves for evaluation. However, their datasets were manually constructed, lacked training sets, and thus fell short in terms of scalability for large-scale applications. While AutoIF \cite{autoif} attempted to address data construction through an automated pipeline, it relied exclusively on code-verifiable constraints, which limits applicability to narrow domains and fails to capture broader, real-world use cases. More critically, most existing datasets impose only a small number of constraints (typically 3–5) and lack systematic evaluation benchmarks or training resources for complex instruction-following tasks. 
Previous automated approaches primarily rely on LLM-based instruction rewriting, which often yields homogenized constraints and limits scalability in generating large numbers of constraints.
Consequently, they are inadequate for rigorously assessing and extending the capability boundaries of LLMs in realistic, complex application settings.

\begin{figure}[]
\centering
\includegraphics[width=0.95 \textwidth]{iclr2026/fig/example.pdf}
\caption{Challenges in complex instruction following and improved performance via RECAST-30k. Left: Real-world examples illustrating how LLMs fail to follow complex instructions. Top-right: Performance degradation of LLMs as the number of constraints increases. Bottom-right: Comparison of instruction-following performance between models fine-tuned on RECAST and their corresponding Instruct variants (e.g., Qwen2.5-7B-Instruct).}
\label{fig:example}
\vspace{-5mm}
\end{figure}


To address these limitations and advance research in this area, we propose RECAST, a scalable data-synthesis framework that constructs instruction-following datasets of unprecedented complexity. Unlike prior approaches, our pipeline systematically mines instruction-following signals from existing data, thereby improving data utilization and fully exploiting the training value of available resources. Through the integration of diverse, verifiable constraints, RECAST enables more rigorous evaluation and more effective enhancement of LLMs’ ability to follow complex instructions.

Based on RECAST, we constructed a high-quality, diverse, and constraint-verifiable dataset, RECAST-30K, which encompasses a large number of constraints spanning diverse types. 
Using only 30K training samples, Llama3.1-8B-Base \cite{llama3} fine-tuned on RECAST-30K already outperforms other instruction-tuning datasets.
Remarkably, it surpasses the corresponding instruct model—trained on a much larger-scale dataset—and even outperforms the substantially larger Llama-3.3-70B-Instruct in handling complex instruction-following scenarios.

Given that the constraints in RECAST-30K can be reliably verified using both rule-based and model-based validators, the dataset is inherently amenable to reinforcement learning. Building on this property, we design RLVC, which further enhances constraint compliance, yielding substantial improvements in multi-constraint satisfaction while preserving general capabilities.

To summarize the highlights of our study:
\begin{itemize}\setlength{\itemsep}{0pt}
    \item We propose \textbf{RECAST}, an efficient, scalable, and low-cost data-synthesis framework that constructs instruction-following datasets of unprecedented complexity, aiming to challenge and enhance state-of-the-art models’ ability to follow complex instructions.

    \item {We release} \textbf{RECAST-30K}, a high-quality dataset purpose-built to benchmark and improve complex instruction-following performance.

    \item {We further exploit the verifiable constraints in RECAST-30K to design} \textbf{RLVC}, a reinforcement-learning approach that leverages constraint-specific reward signals for simultaneous multi-objective optimisation, thereby fully exploiting the supervision potential of the dataset.

\end{itemize}

\section{{R}ealistic {E}xtraction of {C}onstraints for {A}ugmented in{S}truction syn{T}hesis}

\label{headings}

We present RECAST, a comprehensive framework for improving large language models' ability to follow complex, multi-constraint instructions. 
As shown in Figure \ref{fig:main}, the RECAST pipeline operates through a three-stage process. 
First, we construct a rich constraint pool by extracting both rule-based and model-based constraints from seed data. 
Next, we synthesize enhanced instructions by selecting and naturally integrating appropriate constraints into original prompts. Finally, we generate consistent, constraint-compliant responses to these augmented instructions.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99 \textwidth]{fig/main.pdf}

    \caption{Overview of the RECAST framework and RLVC. Left: The RECAST pipeline generates complex instruction-following data through four steps: (1) seed data collection across diverse domains, (2) constraint construction with both rule-based and model-based verification methods, (3) instruction enhancement by integrating selected constraints, and (4) response synthesis ensuring constraints are satisfied. More detailed descriptions of the pipeline are provided in Appendix \ref{appendix:description_of_RECAST}. Top-right: Using RECAST-generated data to fine-tune LLMs through supervised learning. Bottom-right: RLVC framework leveraging constraint-specific verification to provide fine-grained rewards, guiding model optimization toward satisfying multiple constraints simultaneously.}
    \label{fig:main}
\vspace{-3.5mm}
\end{figure}

\subsection{Seed Data Collection}
We select Tülu 3 Persona IF \cite{lambert2024t} as the seed dataset for constructing RECAST-30K. This dataset spans diverse scenarios and task types, including code generation, creative writing, factual question answering, etc., rendering it an appropriate foundation for constraint extraction. A more detailed analysis of the characteristics of this seed dataset is provided in Appendix \ref{sec:seed_dataset_analysis}.


\subsection{Constraint Pool Construction}

To effectively model the multifaceted nature of real-world instructions, we develop a comprehensive constraint pool that captures both objective and subjective requirements. We categorize constraints into two complementary types based on their verification mechanisms, enabling precise assessment of model outputs against diverse criteria.
\textbf{Rule-based Constraints Construction.} Rule-based constraints represent objective requirements that can be verified through deterministic methods, including structural elements (paragraph count), lexical specifications (keyword inclusion/exclusion), and quantitative parameters (word limits). These constraints are particularly valuable as they provide unambiguous verification signals for model training and evaluation.
To systematically extract these constraints, we implement eight specialized rule-based extractors (detailed in Appendix \ref{appendix:taxonomy_rule}) that analyze responses to identify verifiable properties. These extractors recognize specific syntactic patterns, keyword frequencies, numerical parameters, and structural characteristics that can be programmatically verified. This programmatic approach ensures that each rule-based constraint has a corresponding verification method, providing clear training signals for models to learn specific response characteristics.

% \paragraph{Model-based Constraints Construction.}
\textbf{Model-based Constraints Construction.} Model-based constraints encompass subjective requirements that necessitate semantic understanding or qualitative judgment, such as stylistic elements (formality level), tonal qualities (politeness), and content characteristics (persuasiveness). These constraints are crucial for capturing the nuanced aspects of human communication that cannot be reduced to simple rules.
Our construction process follows three key steps: 
First, we analyze each response from the seed datase to determine which constraint types from our taxonomy of 15 categories (detailed in Appendix \ref{appendix:taxonomy_model}) are applicable, ensuring relevance to the specific content. 
Second, we employ LLMs to generate multiple concrete constraint instances for each applicable type, creating a comprehensive initial pool of model-based constraints. 
Third, we implement a filtering process to verify that each constraint is actually satisfied by its corresponding response, removing those that cannot be fulfilled. 
To validate the accuracy of filtering process, we conducted human evaluation on randomly selected constraint-response pairs, confirming that our methodology successfully identifies and retains only appropriate, verifiable constraints (detailed results in Appendix \ref{appendix:human_eval_filter}).

Through this dual-mode construction approach, we create a comprehensive constraint pool that captures both the objective, rule-verifiable aspects and the subjective, semantically-rich dimensions of instruction following. 

\subsection{Constraint-Augmented Instruction Synthesis}
After establishing a verified constraint pool, we develop a three-stage process to create enhanced instructions that effectively incorporate appropriate constraints. This process aims to ensure that the resulting instructions maintain natural language quality while systematically integrating multiple constraints.

\textbf{Constraint Selection.} We employ LLMs to select a coherent subset of constraints from the pool that are relevant and applicable to each original instruction. This selection process ensures that only contextually appropriate constraints are considered for integration, avoiding the inclusion of irrelevant or contradictory requirements.

\textbf{Instruction Enhancement.} Once appropriate constraints are identified, we task multiple LLMs with integrating the selected constraints into the original instruction. Each model produces an enhanced instruction where constraints are incorporated naturally and coherently into the text. 

\textbf{Optimal Instruction Selection.} To ensure quality and consistency, we implement a majority voting mechanism wherein multiple LLMs evaluate and rank the candidate integrated instructions. 
The evaluation criteria include linguistic fluency, semantic coherence, and constraint completeness. 
We select the highest-ranked instruction as the final constraint-augmented instruction. We also performed random sampling on optimal instruction selection for human evaluation, the results of human evaluation are shown in Appendix \ref{appendix:ins_mv}.


\subsection{Instruction-Consistent Response Synthesis}
To address potential inconsistencies between constraint-augmented instructions and original responses in the seed dataset, we implement a two-phase process to ensure alignment while maintaining high response quality.

\textbf{Diverse Response Generation.} We generate multiple candidate responses to each constraint-augmented instruction using distinct LLMs. 
This multi-model approach introduces diversity into the candidate pool and mitigates potential biases inherent to any single model. 
Each model generates responses independently, ensuring a broad representation of possible approaches to satisfying the complex instruction.

% \paragraph{Response Quality Assessment.} 
\textbf{Response Quality Assessment.} We implement a robust majority voting mechanism to evaluate candidate responses based on multiple criteria, including linguistic fluency, factual accuracy, and comprehensive constraint adherence. This systematic evaluation process enables us to identify and select the response that most effectively fulfills all specified requirements while maintaining natural language quality. The winning response becomes part of the final dataset, paired with its corresponding enhanced instruction. To verify the quality of enhanced response, we conducted a human evaluation on randomly sampled instruction-response pairs. The detailed results of this evaluation are presented in Appendix \ref{appendix:res_mv}, confirming the high quality of our selected responses.

This methodical approach to generation and selection ensures that our final dataset comprises constraint-rich and high-quality instruction–response pairs that demonstrate effective navigation of complex, multi-constraint scenarios. Each pair is annotated with its full set of constraints and corresponding validation method, facilitating downstream application and evaluation. 

\section{Reinforcement Learning with Verifiable Constraints as Rewards}
\label{sec:RLwVC}
Since the constraints in RECAST are equipped with corresponding verification methods, the dataset is inherently amenable to reinforcement learning. We therefore introduce RLVC, which leverages the verifiable nature of constraints to provide fine-grained reward signals during policy optimization. Building on SFT-trained models, we further apply RL to maximize the training value of RECAST-30K for enhancing complex instruction-following capabilities. This approach enables more targeted feedback on constraint satisfaction, thereby improving models’ ability to simultaneously address multiple complex requirements.

\subsection{Constraint Verification Mechanisms}
We implement a dual-mode verification scheme that enables precise evaluation of constraint satisfaction. 
Each constraint in an instruction is assessed through either rule-based or LLM-based verification methods.
For rule-based constraints, we employ rule-based validators 
$V_{\text{rule-based}}(x, y, c_i)$ that programmatically verify objective requirements through deterministic procedures. 
For model-based constraints that require evaluation of subjective qualities, we leverage LLM-based validators $V_{\text{model-based}}(x, y, c_i)$. These validators assess more nuanced requirements that resist codification into explicit codes.
We formalize the constraint verification function for an instruction $x$ with response $y$ and constraint $c_i$ as:

{\small
\begin{equation}
  f(x,y,c_i)=\begin{cases}
    V_{\text{rule-based}}(x,y,c_i) & \text{if }c_i\text{ is rule-based}\\
    V_{\text{model-based}}(x,y,c_i) & \text{if }c_i\text{ is model-based}
  \end{cases}
\end{equation}
}


where both verification functions return binary values indicating constraint satisfaction ($1$) or violation ($0$).

\subsection{Verifiable Constraints as Reward Signals}
The key innovation of RLVC lies in its exploitation of RECAST's constraint verifiability feature. 
Traditional reinforcement learning approaches typically rely on a single, holistic reward signal that fails to identify which specific constraints are violated. 
In contrast, RECAST-30K provides individually verifiable constraints, enabling us to design a more informative reward mechanism.
For an instruction $x$ containing multiple constraints $C = \{c_1, c_2, ..., c_n\}$, we define the reward for a generated response $y$ as the average satisfaction rate across all constraints:

\small{
\begin{equation}
\label{eq:reward_func}
R(x, y) = \frac{1}{|C|} \sum_{i=1}^{|C|} f(x, y, c_i)
\end{equation}
 }
 
This design provides an independent reward channel for each constraint, offering fine-grained feedback that guides the model toward simultaneously satisfying multiple constraints.
Our RLVC framework combines verifiable constraints as reward signals with Group Relative Policy Optimization (GRPO) \cite{deepseekmath}. 
Specifically, RLVC leverages the fine-grained feedback enabled by constraint verifiability and optimizes policies via GRPO’s comparative learning approach. 
This integration provides the model with clear guidance on improving constraint satisfaction across diverse instruction types. 
For completeness, we present the detailed formulation of GRPO, including its optimization objective, in Appendix \ref{sec:details_of_rlvc}.

\section{Experiments}
\label{sec:exper}
\subsection{Setups}
\textbf{Evaluation Benchmarks.} We constructed RECAST-Test, a hierarchical evaluation benchmark based on RECAST-30K. This benchmark includes four different difficulty levels, categorized by increasing constraint complexity. Each level comprises instructions with progressively more constraints, enabling fine-grained performance evaluation across tasks of varying complexity. 
More importantly, the number of constraints contained in RECAST-Test far exceeds that of prior benchmarks, making it a more rigorous test of the boundaries of LLMs’ complex instruction-following capabilities. 
The detailed construction method and statistical characteristics of each difficulty level are provided in Appendix \ref{sec:self-eval}.
To assess the generalization and general capabilities of RECAST beyond our constructed benchmark, we further evaluated it on five benchmarks, the details of these benchmarks can be found in Appendix \ref{appendix:general_benchmark}.

% \paragraph{Evaluation Metrics.}
\textbf{Evaluation Metrics.} For evaluation metrics, we use the Hard Constraint Satisfaction Rate (HSR) as the primary metric, quantifying the model's ability to satisfy all specified constraints in an instruction simultaneously. The HSR is calculated as follows:
\small{
\begin{equation}
\text{HSR} = \frac{1}{|D|} \sum_{(x, y) \in D} \prod_{c_i \in C(x)} f(x, y, c_i)
\end{equation}
}

where \(D\) represents the evaluation dataset, \(C(x)\) is the set of constraints for instruction \(x\), and \(f(x, y, c_i)\) is the verification function for constraint \(c_i\).

Additionally, we define the following sub-metrics for different constraint types: (1) \textit{Rule-based Constraint Satisfaction Rate (RSR)}, which measures the HSR score for constraints evaluated using rule-based methods; (2) \textit{Model-based Constraint Satisfaction Rate (MSR)}, which measures the HSR score for constraints evaluated using LLMs; and (3) \textit{Overall Constraint Satisfaction Rate (OSR)}, which quantifies the HSR of all constraints, both rule-based and model-based, that are successfully satisfied simultaneously.
For the FollowBench evaluation, we similarly adopt the Hard Constraint Satisfaction Rate defined in the original benchmark. For all LLM-based evaluations, unless otherwise specified, we default to using GPT-4o \cite{gpt4} for assessment.


% \paragraph{Baselines.}
\textbf{Baselines.} For our baseline comparisons, we primarily select eight high-quality, open-source complex instruction fine-tuning datasets. A detailed description of the baselines can be found in Appendix \ref{sec:baseline}. Additionally, we evaluated the performance of some of the leading large models on the benchmark we constructed.

% \paragraph{Settings.}
\textbf{Settings.} For all experiments, we choose Qwen2.5-7B \cite{qwen2.5} and Llama-3.1-8B \cite{llama3} as the base models. The same experimental setup is used for SFT across all datasets. We use the model after SFT as the base model of RLVC for training. Specific experimental details can be found in Appendix \ref{exp_details}.

\subsection{Main Results}
\renewcommand{\arraystretch}{1.3}

\subsubsection{Evaluation on RECAST-Test}

\begin{table}[t]
\caption{RECAST-Test results across four difficulty levels and overall average. The best result in each column is highlighted in bold, while the second-highest result is indicated with an underline formatting.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|c}
\Xhline{1.5pt}
\multirow{2}{*}{\textbf{Models}}
            & \multicolumn{3}{c|}{\underline{\textbf{Level 1}}}
            & \multicolumn{3}{c|}{\underline{\textbf{Level 2}}}
            & \multicolumn{3}{c|}{\underline{\textbf{Level 3}}}
            & \multicolumn{3}{c|}{\underline{\textbf{Level 4}}}
            & \multirow{2}{*}{\textbf{Average}}\\
            & \textbf{MSR} & \textbf{RSR} & \textbf{OSR}
            & \textbf{MSR} & \textbf{RSR} & \textbf{OSR}
            & \textbf{MSR} & \textbf{RSR} & \textbf{OSR}
            & \textbf{MSR} & \textbf{RSR} & \textbf{OSR} & \\
% \Xhline{1pt}
% \multicolumn{14}{c}{\textbf{Foundation Models}}\\
\Xhline{1pt}
\textbf{Claude-3.7-sonnet} & $90.00$ & $15.50$ & $13.50$ & $86.50$ & $10.00$ & $ 7.00$ & $76.00$ & $ 5.50$ & $ 5.00$ & $60.00$ & $ 6.50$ & $ 4.50$ & $31.67$\\
\textbf{DeepSeek-V3}                &  \underline{$92.50$} & $24.00$ & $21.50$ & $86.50$ & $14.50$ & $11.50$ &  \underline{$81.50$} & $ 9.00$ & $ 7.50$ & $64.00$ & $ 8.50$ & $ 5.00$ & $35.50$\\
\textbf{Gemini-2.5-Pro}   & $91.50$ & \bm{$25.50$} & $22.00$ & \bm{$87.50$} & \bm{$21.00$} & \bm{$19.00$} & $79.00$ & \bm{$16.50$} & \bm{$13.00$} &  \underline{$68.50$} & \bm{$20.00$} & \bm{$13.50$} & \bm{$39.75$}\\
\textbf{GPT-4o}                     & $89.50$ & $24.50$ &  \underline{$22.50$} & $85.00$ & $15.00$ & $10.50$ & $74.50$ & $ 7.50$ & $ 6.00$ & $62.50$ &  \underline{$ 9.00$} &  \underline{$ 7.00$} & $34.46$\\
\textbf{Qwen3-235B-A22B}            & \bm{$96.00$} & \bm{$25.50$} & \bm{$25.00$} &  \underline{$87.00$} & $13.50$ & $10.00$ & \bm{$83.00$} &  \underline{$12.00$} &  \underline{$10.00$} & \bm{$71.00$} & $ 7.00$ & $ 5.50$ &  \underline{$37.13$}\\
\textbf{Qwen2.5-72B-Instruct}       & $88.00$ & $23.50$ & $20.50$ & $79.50$ &  \underline{$16.50$} &  \underline{$12.00$} & $70.00$ & $ 8.50$ & $ 6.50$ & $64.50$ & $ 6.50$ & $ 4.50$ & $33.38$\\
\textbf{Qwen2.5-7B-Instruct}        & $83.50$ & $21.50$ & $18.50$ & $69.00$ & $12.50$ & $ 7.50$ & $51.00$ & $ 3.50$ & $ 2.00$ & $40.50$ & $ 5.00$ & $ 3.00$ & $26.46$\\
\textbf{Llama-3.3-70B-Instruct}     & $79.00$ &  \underline{$25.00$} & $20.00$ & $56.00$ & $14.50$ & $ 9.00$ & $43.00$ & $ 9.00$ & $ 3.00$ & $30.00$ & $ 6.00$ & $ 2.50$ & $24.75$\\
\textbf{Llama-3.1-8B-Instruct}      & $86.50$ & $18.50$ & $15.50$ & $73.00$ & $12.50$ & $ 8.00$ & $53.50$ & $ 8.50$ & $ 4.50$ & $37.00$ & $ 6.00$ & $ 3.50$ & $27.25$\\
\Xhline{1pt}
\multicolumn{14}{c}{\textbf{Llama-3.1-8B}}\\
\Xhline{1pt}
\textbf{Conifer}                    & $73.00$ & $15.00$ & $11.50$ & $54.00$ & $10.00$ & $ 3.00$ & $45.00$ & $ 4.50$ & $ 2.50$ & $32.50$ & $ 0.50$ & $ 0.50$ & $21.00$\\
\textbf{Crab}                       & $59.00$ & $13.00$ & $ 6.00$ & $33.50$ & $ 8.00$ & $ 3.00$ & $24.50$ & $ 3.00$ & $ 0.50$ & $12.00$ & $ 2.50$ & $ 0.50$ & $13.79$\\
\textbf{I-SHEEP}                    & $66.00$ & $14.00$ & $ 8.75$ & $43.75$ & $ 9.00$ & $ 3.00$ & $34.75$ & $ 3.75$ & $ 1.50$ & $22.25$ & $ 1.50$ & $ 0.50$ & $17.40$\\
\textbf{MUFFIN}                & $34.50$ & $ 6.00$ & $ 1.50$ & $19.00$ & $ 4.50$ & $ 2.00$ & $10.00$ & $ 1.00$ & $ 0.00$ & $13.50$ & $ 1.50$ & $ 0.00$ & $ 7.79$\\
\textbf{ShareGPT}                   & $71.00$ & $16.00$ & $10.50$ & $49.00$ & $ 5.00$ & $ 2.00$ & $38.00$ & $ 3.00$ & $ 0.50$ & $27.50$ & $ 2.50$ & $ 1.00$ & $18.83$\\
\textbf{Evol-Instruct}   & $62.50$ & $17.00$ & $10.50$ & $42.50$ & $ 6.50$ & $ 3.00$ & $28.00$ & $ 3.50$ & $ 0.50$ & $20.50$ & $ 2.50$ & $ 1.00$ & $16.50$\\
\textbf{Suri}                       & $ 3.00$ & $ 3.00$ & $ 0.00$ & $ 1.00$ & $ 2.50$ & $ 0.00$ & $ 0.50$ & $ 0.00$ & $ 0.00$ & $ 0.50$ & $ 0.00$ & $ 0.00$ & $ 0.88$\\
\textbf{Tülu 3 Persona IF}&$83.00$&\bm{$22.00$}&\bm{$19.50$}&$70.50$& $9.00$& $5.50$&$55.50$& \underline{$8.00$}& $2.50$&$42.00$& $4.00$& $2.00$&$26.96$\\
\hline
 \rowcolor{pink!30}
\textbf{RECAST-30K-SFT}            & \bm{$86.00$} & \underline{$21.00$} & \underline{$18.50$} & \underline{$78.50$} & \underline{$15.00$} & \underline{$ 9.50$} & \underline{$63.50$} & $ 6.00$ & \underline{$ 4.00$} & \underline{$52.00$} & \underline{$ 8.00$} & \underline{$ 4.50$} & \underline{$30.54$}\\
 \rowcolor{pink!30}
\textbf{RECAST-30K-RLVC}           &  \underline{$83.50$} & \underline{$21.00$} & $17.00$ & \bm{$79.50$} & \bm{$17.50$} & \bm{$12.50$} & \bm{$64.00$} & \bm{$11.50$} & \bm{$7.50$} & \bm{$53.00$} & \bm{$10.00$} & \bm{$6.50$} & \bm{$31.96$}\\
\Xhline{1pt}
\multicolumn{14}{c}{\textbf{Qwen-2.5-7B}}\\
\Xhline{1pt}
\textbf{Conifer}                    & $71.00$ & $16.00$ & $14.00$ & $58.50$ & $ 9.00$ & $ 5.50$ & $45.50$ & $ 6.00$ & $ 3.50$ & $33.50$ & $ 3.00$ & $ 1.00$ & $22.21$\\
\textbf{Crab}                       & $57.50$ & $14.00$ & $ 7.50$ & $30.00$ & $ 7.00$ & $ 3.00$ & $20.50$ & $ 5.00$ & $ 1.00$ & $15.50$ & $ 5.50$ & $ 1.50$ & $14.00$\\
\textbf{I-SHEEP}                    & $56.00$ & $12.50$ & $ 7.50$ & $35.50$ & $ 6.00$ & $ 1.00$ & $26.00$ & $ 3.50$ & $ 0.00$ & $18.00$ & $ 1.50$ & $ 0.00$ & $13.96$\\
\textbf{MUFFIN}                & $61.50$ & $17.00$ & $10.00$ & $46.00$ & $ 7.00$ & $ 4.50$ & $25.50$ & $ 3.50$ & $ 1.00$ & $25.00$ & $ 3.50$ & $ 1.00$ & $17.13$\\
\textbf{ShareGPT}                   & $70.50$ & $13.50$ & $11.00$ & $46.50$ & $ 9.50$ & $ 4.00$ & $34.50$ & $ 3.50$ & $ 2.50$ & $28.00$ & $ 4.50$ & $ 1.50$ & $19.13$\\
\textbf{Evol-Instruct}   & $63.50$ & $14.50$ & $ 8.00$ & $41.00$ & $ 8.00$ & $ 3.00$ & $27.00$ & $ 2.50$ & $ 1.00$ & $22.50$ & $ 4.50$ & $ 2.00$ & $16.46$\\
\textbf{Suri}                       & $ 0.50$ & $ 4.50$ & $ 0.00$ & $ 0.50$ & $ 2.00$ & $ 0.00$ & $ 0.00$ & $ 0.50$ & $ 0.00$ & $ 0.00$ & $ 0.00$ & $ 0.00$ & $ 0.67$\\
\textbf{Tülu 3 Persona IF}&\bm{$88.00$}&\underline{$21.00$}&\bm{$19.50$}&{$69.00$}&$13.00$& $7.00$&$48.50$& $4.50$& $1.50$&$45.00$& $4.00$& $1.00$&$26.83$\\
\hline
 \rowcolor{pink!30}
\textbf{RECAST-30K-SFT}            & \underline{$87.50$} & $18.50$ & $14.50$ & \underline{$76.50$} & \underline{$17.00$} & \bm{$13.00$} & \bm{$66.50$} & \bm{$11.50$} & \bm{$ 6.50$} & \underline{$54.00$} & \underline{$ 5.00$} & \underline{$ 4.50$} & \underline{$31.25$}\\
 \rowcolor{pink!30}
\textbf{RECAST-30K-RLVC}           & $85.50$ & \bm{$22.50$} & \underline{$16.50$} & \bm{$78.00$} & \bm{$19.00$} & \underline{$12.50$} & \underline{$65.50$} & \underline{$10.50$} & \underline{$ 4.50$} & \bm{$55.50$} & \bm{$11.00$} & \bm{$ 7.00$} & \bm{$32.33$}\\
\Xhline{1.5pt}
\end{tabular}}
\label{table:hsr_results}
% \vspace{-8mm}
\end{table}

Table \ref{table:hsr_results} presents comprehensive results from our multi-level constraint satisfaction benchmark. Analysis of these findings reveals three results:

% \paragraph{Performance Degradation with Increasing Constraint Complexity.}
\textbf{Performance Degradation with Increasing Constraint Complexity.} A consistent performance degradation is observed across all models as constraint complexity increases from Level 1 to Level 4. This systematic decline highlights the fundamental challenge LLMs face when processing and satisfying multiple constraints simultaneously. Notably, rule-based constraints present greater difficulties than model-based constraints across all model classes. Among tested models, Gemini-2.5-Pro demonstrates superior constraint handling capabilities with a \bm{$39.75$\%} average satisfaction rate. 
These results underscore that complex instruction following remains a challenging task for current LLMs, and advancing their capabilities in this area is of significant practical importance.

% \paragraph{Effectiveness of RECAST-30K for Instruction Following.}
\textbf{Effectiveness of RECAST-30K for Instruction Following.} Models fine-tuned on RECAST-30K demonstrate substantial improvements in constraint satisfaction capabilities. The RECAST-30K-SFT variant achieves a \bm{$31.25$\%} average satisfaction rate on Qwen-2.5-7B, significantly outperforming both instruction-tuned models and alternative fine-tuning approaches. This enhancement underscores the effectiveness of our constraint-focused dataset in developing robust instruction-following capabilities, particularly for navigating complex, multi-constraint scenarios.

% \paragraph{Performance Enhancement Through RLVC Optimization.}
\textbf{Performance Enhancement Through RLVC Optimization.} The application of RLVC further enhances model performance across all difficulty levels. RECAST-30K-RLVC variants consistently outperform their SFT counterparts, achieving a \bm{$32.33$\%} average satisfaction rate on Qwen-2.5-7B. This improvement is particularly pronounced in higher difficulty levels (Levels 3-4), where constraint interactions become more complex. These gains confirm that our constraint-specific reinforcement learning approach effectively optimizes for simultaneous satisfaction of multiple requirements, addressing a key challenge in practical instruction following.

These results clearly demonstrate that specialized fine-tuning approaches—particularly our RECAST-30K dataset and RLVC optimization framework—significantly enhance LLMs' capability to satisfy multiple complex constraints simultaneously. This improvement addresses a critical gap in current instruction-following systems and enables more reliable performance in constraint-rich applications.


\subsubsection{Evaluation on Additional Instruction-Following Benchmarks.} 
Table \ref{table:instruction_benchmarks} reports results on two widely used instruction-following benchmarks, IFEVAL and FollowBench. RECAST-30K-SFT already surpasses all baseline methods, and RECAST-30K-RLVC further improves performance, achieving the best results on both Llama3.1-8B and QWEN2.5-7B. These consistent gains on out-of-domain benchmarks demonstrate that RECAST not only improves complex constraint-following but also generalizes effectively to traditional instruction-following tasks, rather than merely overfitting to the constraint patterns seen during training.

\begin{table}
\centering
\caption{Results on instruction-following benchmarks (IFEVAL and FollowBench). IFEVAL uses Prompt-Level Loose Accuracy (\textit{Pr. (L)}), while FollowBench uses Hard Satisfaction Rate (\textit{HSR}). The best result in each column is highlighted in bold, while the second-highest result is indicated with underline formatting.}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|cc|c|cc|c}
\Xhline{1.5pt}
\multirow{3}{*}{\textbf{Models}} 
& \multicolumn{2}{c|}{\underline{\textbf{Llama3.1-8B}}} 
& \multirow{3}{*}{\textbf{Avg.}} 
& \multicolumn{2}{c|}{\underline{\textbf{QWEN2.5-7B}}} 
& \multirow{3}{*}{\textbf{Avg.}} \\
& \textbf{IFEVAL} & \textbf{Followbench} & 
& \textbf{IFEVAL} & \textbf{Followbench} & \\
& \textit{Pr. (L)} & \textit{HSR} & 
& \textit{Pr. (L)} & \textit{HSR} & \\
\Xhline{1pt}
\textbf{Conifer}           & $43.62$ & $44.69$ & $44.16$ & $44.73$ & $52.27$ & $48.50$ \\
\textbf{Crab}              & $42.14$ & $41.90$ & $42.02$ & $44.55$ & $44.50$ & $44.53$ \\
\textbf{I-SHEEP}           & $32.90$ & $29.48$ & $31.19$ & $36.60$ & $35.38$ & $35.99$ \\
\textbf{MUFFIN}            & $24.95$ & $16.78$ & $20.87$ & $36.78$ & $42.15$ & $39.47$ \\
\textbf{ShareGPT}          & $46.40$ & $45.41$ & $45.91$ & $47.13$ & $49.06$ & $48.10$ \\
\textbf{Evol-Instruct}     & $42.70$ & $36.60$ & $39.65$ & $45.29$ & $46.34$ & $45.82$ \\
\textbf{Suri}              & $18.30$ & $4.02$  & $11.16$ & $12.75$ & $5.59$  & $9.17$ \\
\textbf{Tülu 3 Persona IF} & $73.94$ & $55.44$ & $64.69$ & \underline{$73.94$} & $56.94$ & $65.44$ \\
\hline
\rowcolor{pink!30}
\textbf{RECAST-30K-SFT}    & \underline{$76.34$} & \underline{$57.10$} & \underline{$66.72$} & $73.38$ & \underline{$59.60$} & \underline{$66.49$} \\
\rowcolor{pink!30}
\textbf{RECAST-30K-RLVC}   & \bm{$77.39$} & \bm{$61.76$} & \bm{$69.58$} & \bm{$74.01$} & \bm{$63.23$} & \bm{$68.62$} \\
\Xhline{1.5pt}
\end{tabular}
}
\label{table:instruction_benchmarks}
\end{table}

\subsubsection{General Capability Evaluation}

\begin{table}[t]
\centering
\caption{Results on general capability benchmarks (GPQA and MUSR). All metrics use standard Accuracy (\textit{Acc}), measuring the percentage of correct responses. The best result in each column is highlighted in bold, while the second-highest result is indicated with underline formatting.}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{l|cc|c|cc|c}
\Xhline{1.5pt}
\multirow{3}{*}{\textbf{Models}} 
& \multicolumn{2}{c|}{\underline{\textbf{Llama3.1-8B}}} 
& \multirow{3}{*}{\textbf{Avg.}} 
& \multicolumn{2}{c|}{\underline{\textbf{QWEN2.5-7B}}} 
& \multirow{3}{*}{\textbf{Avg.}} \\
& \textbf{GPQA} & \textbf{MUSR} & 
& \textbf{GPQA} & \textbf{MUSR} & \\
& \textit{Acc} & \textit{Acc} & 
& \textit{Acc} & \textit{Acc} & \\
\Xhline{1pt}
\textbf{Conifer}           & $27.61$ & $37.64$ & $32.63$ & $31.22$ & $45.54$ & $38.38$ \\
\textbf{Crab}              & \bm{$32.48$} & \underline{$40.26$} & $36.37$ & \underline{$31.89$} & \bm{$48.74$} & \bm{$40.32$} \\
\textbf{I-SHEEP}           & $28.33$ & $36.30$ & $32.32$ & $29.95$ & $43.18$ & \underline{$36.57$} \\
\textbf{MUFFIN}            & $26.64$ & $33.69$ & $30.17$ & $29.07$ & $37.93$ & $33.50$ \\
\textbf{ShareGPT}          & $30.02$ & $40.16$ & \underline{$35.09$} & $31.20$ & $44.95$ & $38.08$ \\
\textbf{Evol-Instruct}     & $28.41$ & \bm{$41.75$} & \bm{$35.08$} & \bm{$32.55$} & \underline{$47.41$} & $39.98$ \\
\textbf{Suri}              & $26.09$ & $33.40$ & $29.75$ & $26.60$ & $41.79$ & $34.20$ \\
\textbf{Tülu 3 Persona IF} & $28.64$ & $38.68$ & $33.66$ & $31.06$ & $44.13$ & $37.60$ \\
\hline
\rowcolor{pink!30}
\textbf{RECAST-30K-SFT}    & $26.77$ & $37.39$ & $32.08$ & $30.02$ & $39.91$ & $34.97$ \\
\rowcolor{pink!30}
\textbf{RECAST-30K-RLVC}   & \underline{$30.81$} & $38.47$ & $34.64$ & $29.84$ & \underline{$46.94$} & $38.39$ \\
\Xhline{1.5pt}
\end{tabular}
}
\label{table:general_benchmarks}
\end{table}

In addition, we evaluate RECAST on two general capability benchmarks (Table~\ref{table:general_benchmarks}), where RECAST-30K-RLVC achieves average scores of $34.64$ on Llama3.1-8B and $38.39$ on QWEN2.5-7B. This indicates that while RECAST substantially improves performance on complex instruction following, it also preserves competitive performance on reasoning-oriented benchmarks like MUSR and knowledge-focused evaluations such as GPQA.

\section{Related Work}
\label{gen_inst}

\textbf{Complex Instruction Datasets Construction. }Recent research has explored various approaches to automatically construct complex instruction datasets. WizardLM \cite{xu2024wizardlm} introduced Evol-Instruct, which iteratively increases instruction difficulty through rewriting. Conifer \cite{sun2024conifer} employs a top-down approach using GPT-4 to generate multi-level constraint instructions. ULTRAIF \cite{an2025ultraif} decomposes instructions into basic queries and constraints before recombination, while AIR \cite{liu2025air} applies an iterative refinement framework that progressively adds constraints through a model-judge cycle. Other approaches include MUFFIN \cite{lou2023muffin}, which builds multi-faceted tasks by expanding input features, and CRaB \cite{crab}, which infers new constraints from existing instruction-response pairs through back-translation. Unlike these methods, our RECAST approach uniquely focuses on mining diverse constraint types from responses in the seed dataset and incorporates explicit verification mechanisms for both rule-based and model-based constraints, addressing limitations in existing methods regarding constraint complexity, diversity, and quality assurance.

\textbf{Complex Instruction Following Capabilities Improvement.} Recent algorithmic innovations have significantly advanced instruction following capabilities. AutoIF \cite{autoif} implements a self-dialogue generation process with execution-based verification, filtering training data through executable feedback. RNR \cite{rnr} extracts roles and rules from existing instructions to generate rule-compliant responses, while SPaR \cite{spar} employs self-play tree search refinement through multiple rounds of model self-adversarial interaction to optimize response quality. The approach in \cite{From_Complex_to_Simple} utilizes discriminative generation, applying a discriminator model to filter generated samples for higher-quality supervision. 

Unlike prior approaches, our method leverages the verification methods in RECAST-30K that encompass both quantitative and qualitative constraints, maximizing its supervisory potential beyond Supervised Fine-Tuning by designing multi-channel reward signals that treat each constraint as an independent optimization objective for RLVC training, thereby leading to significant gains in both the accuracy and consistency of complex instruction following.


==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

